Convective quenching of stellar pulsations

Context: we study the convection-pulsation coupling that occurs in cold Cepheids close to the red edge of the classical instability strip. In these stars, the surface convective zone is supposed to stabilise the radial oscillations excited by the kappa-mechanism. Aims: we study the influence of the convective motions onto the amplitude and the nonlinear saturation of acoustic modes excited by kappa-mechanism. We are interested in determining the physical conditions needed to lead to a quenching of oscillations by convection. Methods: we compute two-dimensional nonlinear simulations (DNS) of the convection-pulsation coupling, in which the oscillations are sustained by a continuous physical process: the kappa-mechanism. Thanks to both a frequential analysis and a projection of the physical fields onto an acoustic subspace, we study how the convective motions affect the unstable radial oscillations. Results: depending on the initial physical conditions, two main behaviours are obtained: (i) either the unstable fundamental acoustic mode has a large amplitude, carries the bulk of the kinetic energy and shows a nonlinear saturation similar to the purely radiative case; (ii) or the convective motions affect significantly the mode amplitude that remains very weak. In this second case, convection is quenching the acoustic oscillations. We interpret these discrepancies in terms of the difference in density contrast: larger stratification leads to smaller convective plumes that do not affect much the purely radial modes, while large-scale vortices may quench the oscillations.

==> Makefile <==
# $Id: Makefile,v 1.3 2010/06/22 13:11:55 tgastine Exp $
# Makefile for generating different output formats of the $(FILE) inspired
# from the Pencil Code one used to build the manual.
#
# Usage:
#  make
#  make $(FILE).pdf
#  make clean
#
# ------------------
FILE             = paper
LATEX            = latex -src
DVIPS            = dvips
BIBTEX           = bibtex
PS2PDF           = ps2pdf14 -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress
MAY_HAVE_CHANGED = 'may have changed. Rerun to get'
MAY_NO_BIBTEX    = 'undefined citations'
# ------------------
.SUFFIXES:            # clear all generic rules and suffixes
.SUFFIXES: .tex .dvi .ps .pdf

.tex.dvi:
	$(LATEX) $*
	if [ `fgrep -c $(MAY_HAVE_CHANGED) $*.log` != '' ]; then \
	    $(LATEX) $*; \
	fi
.dvi.ps:
	$(DVIPS) $* -o $*.ps
.ps.pdf:
	$(PS2PDF) $*.ps $*.pdf
# ------------------

default: $(FILE).ps

all: $(FILE).ps $(FILE).pdf

$(FILE).dvi: $(FILE).tex
	@TEXINPUTS="./texinputs:${TEXINPUTS}"; \
	export TEXINPUTS; \
	echo "TEXINPUTS=$${TEXINPUTS}"; \
	$(LATEX) $(FILE) \
	    && if [ `fgrep -c $(MAY_HAVE_CHANGED) $(FILE).log` != '' ]; then \
	           $(LATEX) $(FILE); \
	       fi \
	    && if [ `fgrep -c $(MAY_NO_BIBTEX) $(FILE).log` != '' ]; then \
	    $(BIBTEX) $(FILE); \
	    $(LATEX) $(FILE); \
	    $(LATEX) $(FILE); \
	       fi

$(FILE).pdf: $(FILE).ps
	$(PS2PDF) $(FILE).ps

$(FILE).ps: $(FILE).dvi
	$(DVIPS) $(FILE) -o $(FILE).ps

bib:
	bibtex $(FILE)

# Clean up
clean:
	rm -f $(FILE).ps* $(FILE).dvi *.aux *.toc *.log *.bbl *.blg \
	$(FILE).pdf $(FILE).out

# End of file
# dependencies:
$(FILE).dvi: fig/*.eps
$(FILE).dvi: *.bib

